CMB-S4 Technology Book, First Edition

CMB-S4 is a proposed experiment to map the polarization of the Cosmic Microwave Background (CMB) to nearly the cosmic variance limit for angular scales that are accessible from the ground. The science goals and capabilities of CMB-S4 in illuminating cosmic inflation, measuring the sum of neutrino masses, searching for relativistic relics in the early universe, characterizing dark energy and dark matter, and mapping the matter distribution in the universe have been described in the CMB-S4 Science Book. This Technology Book is a companion volume to the Science Book. The ambitious science goals of CMB-S4, a "Stage-4" experiment, require a step forward in experimental capability from the current Stage=II experiments. To guide this process, we summarize the current state of CMB instrumentation technology, and identify R&D efforts necessary to advance it for use in CMB-S4. The book focuses on technical challenges in four broad areas: Telescope Design; Receiver Optics; Focal-Plane Optical Coupling; and Focal-Plane Sensor and Readout.

==> Introduction/acronym_intro.tex <==
%\documentclass[a4paper]{article}
%\begin{document}
%\subsection*{Acronyms}
%
%%Introduction
\begin{flushleft}
\begin{tabular} {ll}
\textbf{CD} & Critical Decision \\
\textbf{MSQUID} & Microwave Superconducting Quantum Interference Device \\
\textbf{PSL} &  Production Status Level \\
\textbf{TSL} &  Technology Status Level\\
\textbf{WIMP} & Weakly Interacting Massive Particles \\
\end{tabular}
\end{flushleft}
%
%\end{document} 


==> Makefile <==
TARGET := cmbs4_instbook
MKPATH := $(shell dirname $(abspath $(lastword $(MAKEFILE_LIST))))

# file extensions `make clean` will delete with impunity ; use with care
AUX_EXTENSIONS := aux log out toc bbl blg

all:  
	pdflatex $(TARGET)
# the - at the beginning of this line instructs the Makefile to ignore errors from bibtex and continue compiling.
# necessary right now because the bibliography has a whole bunch of errors.
	-bibtex $(TARGET)
	pdflatex $(TARGET)
	pdflatex $(TARGET)
#       dvips -o $(TARGET).ps -t letter $(TARGET).dvi


clean:
# remove all auxiliary files
	for ext in $(AUX_EXTENSIONS) ; do \
		find $(MKPATH) -name "*.$$ext" -exec rm -v {} \; ; \
	done

==> abstract.tex <==
CMB-S4 is a proposed experiment to map the polarization of the Cosmic Microwave Background (CMB) to nearly the cosmic variance limit for the angular scales that are accessible from the ground. The science goals and capabilities of CMB-S4 in illuminating cosmic inﬂation, measuring the sum of neutrino masses, searching for relativistic relics in the early universe, characterizing dark energy and dark matter, and mapping the matter distribution in the universe have been described in the CMB-S4 Science Book.
This Technology Book is a companion volume to the Science Book.  The ambitious science goals of the proposed Stage-IV’ CMB-S4 will require a step forward in experimental capability from the current Stage-III experiments. To guide this process, the community summarized the current state of the technology and identify R&D eﬀorts necessary to advance it for possible use in CMB-S4. The book focused on the technical challenges in four broad areas: Telescope Design; Receiver Optics; Focal-Plane Optical Coupling; and Focal-Plane Sensors and Readout. 

==> acronym_execsumm.tex <==
%\documentclass[a4paper]{article}
%\begin{document}
%\subsection*{Acronyms}
%
%
%% executive summary
\begin{flushleft}
\begin{tabular} {ll}
%\textbf{ANL} & Argonne National Laboratory \\
\textbf{AR} & Anti-Reflection (Coating) \\
\textbf{CMB} & Cosmic Microwave Background \\
%\textbf{DOE} & Department of Energy \\
\textbf{FDM} & Frequency Division Multiplexing \\
\textbf{HWP} & Half-Wave Plate \\
\textbf{IR} & InfraRed \\
%\textbf{LBNL} & Lawrence Berkeley National Laboratory \\
\textbf{MKID} & Microwave Kinetic Inductance Detector \\
\textbf{PSL} & Production Status Level \\
\textbf{PTFE} & PolyTetraFluoroEthylene \\
\textbf{R\&D} & Research and Development \\
%\textbf{SLAC} & Stanford Linear Accelerator Center \\
\textbf{SQUID} & Superconducting Quantum Interference Device \\
\textbf{TDM} & Time Division Multiplexing \\
\textbf{TES} & Transition Edge Sensor \\
\textbf{TSL} & Technology Status Level \\
\end{tabular}
\end{flushleft}
%
%\end{document}


==> broadband_optics/acronym_optics.tex <==
%\documentclass[a4paper]{article}
%\begin{document}
%\subsection*{Acronyms}
%%optics
%
\begin{flushleft}
\begin{tabular} {ll}
%\textbf{3-D} & Tridimensional \\
\textbf{ADM} & Artificial Dielectric Material \\
\textbf{AHWP} & Achromatic Half Wave Plate \\
\textbf{AR} & Anti-Reflection \\
\textbf{ARC} &  Anti-Reflection Coating \\
\textbf{BOPP} & Biaxially Oriented Polyproylene \\
\textbf{CHES} &  Controlled Heat Extraction System \\
%\textbf{CMB} & Cosmic MIcrowave Background \\
\textbf{CMM} &  Coordinate Measuring Machine\\
\textbf{CNC} & Computer Numerical Control\\
\textbf{CTE} & Coefficient of thermal expansion\\
\textbf{DRIE} & Deep Reactive Ion Etching \\
\textbf{EFG} &  Edge-deﬁned Film-fed Growth  \\
\textbf{FIR} & FarInfraRed\\
\textbf{FP} & Fabry-Perot \\
\textbf{FTS} & Fourier Transform Spectrometer\\
\textbf{HDPE} & High-Density PolyEthylene \\
\textbf{HEM} & Heat Exchanger Method \\
\textbf{HF} & High Frequency \\
\textbf{HWP} & Half Wave Plate \\
\textbf{IGW} & Inflationary Gravitational Waves \\
\textbf{IR} & InfraRed \\
\textbf{JFET} & Junction gate Field-Effect Transistor \\
\textbf{LAIS} & Laser Ablated Infrared Shaders \\
\textbf{LDPE} & Low-Density PolyEthylene \\
\textbf{LED} & Light-Emitting Diode \\
\textbf{LF} & Low Frequency \\
%\textbf{LHE} & Liquid Helium \\
\textbf{MF} & Medium Frequency \\
\textbf{MMF} & Metal Mesh Filter \\
%\textbf{N2} & Nitrogen \\
\textbf{NIR} & Near InfraRed\\
\textbf{NTD} & Neutron Transmutation Doped \\
\textbf{PPTFE} & Porous PolyTetraFluoroEthylene \\
\textbf{PSL} & Production Status Level \\
\textbf{PTFE} & PolyTetraFluoroEthylene\\
\textbf{QWP} & Quarter Wave Plate\\
\textbf{R\&D} & Research and Development \\
\textbf{RT-MLI} & Radio-Transparent Multi-Layer Insulation \\
\textbf{SMB} & Superconducting Magnetic Bearings \\
\end{tabular}
\end{flushleft}

\clearpage
\begin{flushleft}
\begin{tabular} {ll}
\textbf{SWS} & SubWavelength Structures \\
%\textbf{TMM} & \comred{???}  \\
\textbf{TOD} & Time Ordered Data \\
\textbf{TSL} & Technology Status Level \\
\textbf{UHMWPE} & Ultra-High Molecular Weight PolyEthylene \\
\textbf{VNA} & Vector Network Analyzer \\
\textbf{VPM} & Variable Polarization Modulator \\
\end{tabular}
\end{flushleft}
%
%\end{document} 


==> detector_rf/Conclusion.tex <==
Multichroic detector offers attractive solution to frequency bandwidth and frequency resolution demands of CMB-S4 to characterizing astrophysical foreground.
Broadband antenna increases optical throughput of a single detector by covering wide frequency range, and a multiplexing RF filter partitions broadband signal into narrow frequency bands.
Selecting resolution and bandwidth of a pixel is a complex global optimization challenge that requires collaborative work between forecast team and instrument team.

Multi-chroic detector technologies are getting mature with current CMB experiments.
Broadband horn demonstrated 2.2:1 bandwidth, and lenslet coupled sinuous antenna demonstrated 5:1 bandwidth. 
Both antennas demonstrated round beam and polarization leakage at percent level.
Quad-ridged horn feed is being developed to extend horn bandwidth to 6:1 bandwidth.
Broadband antenna array that can achieve an octave bandwidth is also in development. 

Scaling up detector fabrication for CMB-S4 requires increase in production throughput.
Expertise in large scale deployment from national laboratories will be essential, and appropriate technologies can be outsourced to an industry micro-fabrication facility to increase throughput. 
Also emerging technologies such as metamaterial lenslet array may facilitate mass production in addition to potential performance boost.

RF engineering techniques to CMB applications is now a mature technology.
Techniques were successfully implemented in Stage-2 and upcoming Stage-3 experiments.
Coupling RF signal to both TES bolometer and MKID were demonstrated.
Broadband pixels with diplexer and triplexer band pass filters are deploying with Stage-3 experiments. 
Seven channel channelizer filter band was demonstrated, and high resolution filter banks are in development for both TES bolometer and MKID coupling.
Low loss transmission line is essential for boosting detector efficiency and providing flexibility in the circuit design.
Silicon oxide, silicon nitride, and single crystal silicon dielectric films were explored.
Silicon nitride and single crystal silicon have low loss-tangents that are attractive for detector design. 
With low loss transmission line, implementing higher order filter becomes feasible.
For potential desire to subdivide atmospheric band, higher order filter will give degree of freedom needed for detector designer to use a filter with sharp roll off without inquiring undesirable loss.
Stable material property is important for predictable RF performance.
Fabrication facility that has stable environment is necessary for mass production of detectors with predictable performance.

Ground based experiment tends to favor small pixel size for the optimal mapping speed.
This contradicts with desire to increase number of bands on a single pixel as number of components on a detector wafer increases.
For a potentially denser detector array for CMB-S4, there are multiple development happening to address packaging issue. 
Wire bonds can be made in multiple tiers to effectively multiply available perimeter space for wire bonding.
CMB experiments are already using two tier wire bonding, but micro-fabrication industry can easily do 4 tiers or more.
It is also possible to reduce number of wire bond by integrating by multiplexing readout circuit on a wafer.
As readout frequency range for a next generation readout architecture approaches $\sim$100~MHz to $\sim$1~GHz, multiplexing resonators becomes small enough that it can be integrated with detectors on a single wafer.
This approach simplifies integration of an entire system and allow tighter control of parasitic impedances.
Also a new telescope design used by the Advanced ACTPol that physically separates adjacent detector arrays gives more freedom in detector array design. 

Detector characterization is an essential part of detector fabrication.
Timely feedback with accurate information is important for a successful iteration to fabricate high performance detector. 
Multiple institutions already have detector test setups and experience to characterize detector array. 
However, development is required to meet demands for higher detector throughput of CMB-S4.
Automation of detector characterization would be necessary to increase detector testing throughput.
Also differences between test setups make comparison of results difficult.
Standard test setups and methods should be established to characterize detector arrays at different institutions.
Systematics requirement on RF performance will be tighter for a more sensitive future CMB experiment. 
Detector characterization need to be able to characterize a detector with high accuracy to meet these requirements. 

Multichroic detectors are deploying in field, and new ideas are being tested in laboratories.
Diverse designs have unique strength and short comings. 
Systematics that arise from non-idealities in detector performance and cost evaluation were not addressed in this technical paper. 
For next iteration of the technical paper, both topics should be included.
Detector RF design will be chosen based on a global optimization that would maximize science result.




==> detector_rf/Intro_Goal.tex <==
\subsection{Goal of CMB-S4 technical papers}
\label{sec:goal}
Summarize the current state of the technology and identify R\&D efforts necessary to advance it for possible use in CMB-S4. CMB-S4 will require a scale-up in number of elements, frequency coverage, and bandwidth relative to current instruments. Because it is searching for lower magnitude signals, it will also require stronger control of systematic uncertainties.  


==> detector_rf/acronym_RFdet.tex <==
%\documentclass[a4paper]{article}
%\begin{document}
%\subsection*{Acronyms}
%
%%detector RF
\begin{flushleft}
\begin{tabular} {ll}
%\textbf{AdvACT} & Advanced Atacama Cosmology Telescope \\
\textbf{ADR} & Adiabatic Demagnetization Refrigerator  \\
\textbf{AR} & AntiReflection \\
\textbf{BUG} & Backshort-Under-Grid \\
\textbf{CAD} & Computer-Aided Design\\
\textbf{CNC} & Computer Numeric Control \\
\textbf{CWG} & Continuous Wave guide \\ 
\textbf{CPW} & Co-Planar Wave guide \\
%\textbf{CU} & University of Colorado Boulder \\
\textbf{DfMUX} & Digital frequency Multiplexing\\
\textbf{DRIE} & Deep Reactive Ion Etching \\
\textbf{EM} & electromagnetic \\
\textbf{FNL} & Fermi National Laboratory \\
\textbf{FTS} & Fourier Transform Spectrometer\\
\textbf{GRIN} & GRadient-INdex \\
\textbf{HWP} & Half Wave Plate \\
\textbf{IDC} & interdigitated capacitors \\
\textbf{IR} & InfraRed \\
\textbf{KID} & Kinetic Inductance Detector \\
%\textbf{LBNL} & Lawrence Berkeley National Laboratory\\
\textbf{LEKID} & Lumped-Element Kinetic Inductance Detector \\
%\textbf{MBAC} & Millimeter Bolometric Array Camera \\
\textbf{MEM} &  Micro-ElectroMechanical \\
\textbf{MKID} & Microwave Kinetic Inductance Detector \\
\textbf{MSQUID} & Micorwave Superconducting Quantum Interference Device \\
\textbf{NEP} & Noise Equivalent Power \\
%\textbf{NIST} & National Institute of Standards and Technology \\
\textbf{OMT} & Ortho-Mode Transducer \\
\textbf{PSL} & Production Status Level  \\
\textbf{PTCs} & Pulse-Tube Coolers \\
\textbf{PTFE} & PolyTetraFluoroEthylene \\
\textbf{RF} & Radio Frequency \\
%\textbf{RMS} & Root mean square \\
\textbf{SOI} & Silicon-on-Insulator \\
\textbf{SQUID} & Superconducting Quantum Interference Device \\
\textbf{Tc} & Critical Temperature\\
\textbf{TES} & Transition Edge Sensor\\
\textbf{TL} & Transmission Line \\
\textbf{TSL} & Technology Status Level \\
\textbf{UHMWPE} & Ultra-High Molecular Weight PolyEthylene \\
\textbf{VNA} & Vector Network Analyzer \\
\end{tabular}
\end{flushleft}
%
%\end{document} 


==> endorsers/authors.tex <==
Maximilian	H.	Abitbol,
Zeeshan		Ahmed,
Darcy		Barron,
Ritoban		Basu Thakur,
Amy	N.	Bender,
Bradford	A.	Benson,
Colin	A.	Bischoff,
Sean	A.	Bryan,
John	E.	Carlstrom,
Clarence	L.	Chang,
David	T.	Chuss,
Ari		Cukierman,
Tijmen		de Haan,
Matt		Dobbs,
Tom		Essinger-Hileman,
Jeffrey	P.	Filippini,
Ken		Ganga,
Jon	E.	Gudmundsson,
Nils	W.	Halverson,
Shaul		Hanany,
Shawn	W.	Henderson,
Charles	A.	Hill,
Shuay-Pwu	P.	Ho,
Johannes		Hubmayr,
Kent		Irwin,
Oliver		Jeong,
Bradley	R.	Johnson,
Sarah	A.	Kernasovskiy,
John	M.	Kovac,
Akito		Kusaka,
Adrian	T.	Lee,
Salatino		Maria,
Philip		Mauskopf,
Jeff	J.	McMahon,
Lorenzo		Moncelsi,
Andrew	W.	Nadolski,
Johanna	M.	Nagy,
Michael	D.	Niemack,
Roger	C.	O'Brient,
Stephen		Padin,
Stephen	C.	Parshley,
Clement		Pryke,
Natalie	A.	Roe,
Karwan		Rostem,
John		Ruhl,
Sara	M.	Simon,
Suzanne	T.	Staggs,
Aritoki		Suzuki,
Eric	R.	Switzer,
Keith	L.	Thompson,
Peter		Timbie,
Gregory	S.	Tucker,
Joaquin	D.	Vieira,
Abigail	G.	Vieregg,
Benjamin		Westbrook,
Edward	J.	Wollack,
Ki Won		Yoon,
Karl	S.	Young,
Edward	Y.	Young

==> readout/acronym_readout.tex <==
%\documentclass[a4paper]{article}
%\begin{document}
%\subsection*{Acronyms}
%
%%Readout
\section*{List of acronyms}

\begin{flushleft}
\begin{tabular} {ll}

%\textbf{ABS} & Atacama B modes search\\
%\textbf{AC} & \\
%\textbf{ACT} & Atacama Cosmology Telescope\\
\textbf{ADC} & Analog to Digital Converter \\
%\textbf{AdvACT} & Advanced Atacama Cosmology Telescope\\
%\textbf{AMKID}& \\
%\textbf{APEX}& Atacama Pathfinder EXperiment\\
%\textbf{AWG} &\\
%\textbf{BLAST}& Balloon-borne Large Aperture Submillimeter Telescope\\
%\textbf{BLAST}& TNG \\
%\textbf{CMB}& Cosmic Microwave Background\\
\textbf{CDM} & Code-Division Multiplexing \\
%\textbf{CHIME}&The Canadian Hydrogen Intensity Mapping Experiment\\
%\textbf{CLASS}&Cosmology Large Angular Scale Surveyor\\
\textbf{CPW} & Co-Planar Wave guide \\
%\textbf{CSO} & Caltech Submillimeter Observatory \\
\textbf{DAC} & Digital to Analog Converter \\
\textbf{DAN} & Digital Active Nulling \\
%\textbf{DC}&\\
%\textbf{DfMUX}&\\
%\textbf{DOE} & Department of Energy \\
%\textbf{EBEX}& E and B Experiment\\
%\textbf{EPIC-IM}& \\
\textbf{ESR}& Equivalent Series Resistance\\
\textbf{FDM} & Frequency Division Multiplexing\\
\textbf{FIR}& Finite Impulse Response filter\\
\textbf{FPGA} &  Field-Programmable Gate Array \\
%\textbf{GBT} & Green Bank Telescope \\
\textbf{HEMT} & High-Electron Mobility Transistor \\
%\textbf{ICE}&\\
\textbf{IF} &  Intermediate Frequency  \\
\textbf{IFFT}& Inverse Fast Fourier Transform\\
\textbf{IQ} & In-phase and quadrature phase \\
%\textbf{IRAM}&\\
\textbf{KID} & Kinetic Inductance Detector \\
%\textbf{LC}&\\
\textbf{LCLS-II} & Linac Coherent Light Source II  \\
%\textbf{LCR}&\\
\textbf{LEKID} & Lumped-Element Kinetic Inductance Detector \\
\textbf{LNA} & Low Noise Amplifier \\
\textbf{LO} & Local Oscillator\\
%\textbf{MAKO}&\\
\textbf{MCE} & Multi-Channel Electronics \\
\textbf{MEMS}& MicroElectroMechanical System\\
\textbf{MKID} & Microwave Kinetic Inductance Detector \\
\textbf{MOS} & metal-oxide-semiconductor \\
%\textbf{MUSIC}& MUlticolor Sub/millimeter Inductance Camera\\
%\textbf{MUX} &\\
\textbf{NEP} & Noise Equivalent Power\\
\textbf{NET} & Noise Equivalent Temperature \\
%\textbf{NIKA}&\\
%\textbf{NIKA2}&\\
%\textbf{NIST} & National Institute of Standards and Technology \\
%\textbf{PB}& \\
%\textbf{PID}&\\
\textbf{PSL}& Production Status Level\\
%\textbf{QUBIC}&\\
%\textbf{RC}&\\
\textbf{RFI} & Radio Frequency Interference\\
%\textbf{RF-SQUID} & Radio Frequency Superconducting Quantum Interference Device \\
%\textbf{RLC} & resonant circuit \\
%\textbf{ROACH}&Reconfigurable Open Architecture Computing Hardware\\
\textbf{RRR}&  Residual Resistivity Ratio\\
%\textbf{RMS} & Root Mean Square \\
%\textbf{SCUBA}&\\
%\textbf{SPT}& South Pole Telescope\\
\textbf{SOI} & Silicon On Insulator \\
\textbf{SQ1} & first-stage SQUID \\
%\textbf{SRON}& \\
\textbf{SSA} & Series SQUID Array \\
\textbf{SQUID} & Superconducting Quantum Interference Device \\
\textbf{Tc} & critical Temperature \\
\textbf{TDM} & Time Division Multiplexing \\
\textbf{TES} & Transition Edge Sensor \\
\textbf{TiN}& Titanium Nitride \\
\textbf{TLS} & Two-Level System \\
\textbf{TSL}& Technology Status Level\\
%\textbf{UBC} & University British Columbia \\
\textbf{\umux{}} & microwave SQUID multiplexer \\
\end{tabular}
\end{flushleft}
%
%\end{document} 


==> readout/packages.tex <==
\usepackage{amssymb,amsmath,graphicx,times,epsfig}
\usepackage{fullpage}
\usepackage{lineno}
\usepackage{hyperref}
\usepackage{color}
\usepackage{lscape}
\graphicspath{{figures/}}

% TDM
\numberwithin{equation}{section}
\usepackage[utf8]{inputenc}
\usepackage{xspace}
\newcommand{\ie}{{\it i.e.}\xspace}
\newcommand{\eg}{{\it e.g.}\xspace}
\newcommand{\etal}{{\it et al.}\xspace}
\newcommand{\spider}{{\sc Spider}\xspace}
\newcommand{\ebex}{{\sc EbEx}\xspace}
\newcommand{\piper}{{\sc Piper}\xspace}
\newcommand{\litebird}{Lite{\sc Bird}\xspace}
\newcommand{\polarbear}{{\sc Polarbear}\xspace}
\newcommand{\planck}{{\it Planck}\xspace}
\newcommand{\bicep}{{\sc Bicep}\xspace}
\newcommand{\biceptwo}{{\sc Bicep}2\xspace}
\newcommand{\bicepthree}{{\sc Bicep}3\xspace}

%bib
\newcommand{\apj}{Astrophys. J.}
\newcommand{\apjl}{Astrophys. J. Lett.}
\newcommand{\apjs}{Astrophys. J. Supp.}
\newcommand{\prd}{Phys. Rev. D.}
\newcommand{\aap}{Astron. and Astroph.}
\newcommand{\nat}{Nature}
\newcommand{\mnras}{Mon. Not. R. Astron. Soc.}
\newcommand{\procspie}{Proc. SPIE}



==> tcilcomm.tex <==
% Macros used for TCI styles released with Scientific Word 1.1.
%Copyright (C) 1992-93 TCI Software Research, Inc.
\typeout{TCILCOMM Macros for TCI styles <08 Apr 93>.}
%
% Revisions:
% 08 Apr 93 - GP change line length to under 80 characters
% 30 Mar 92 - AO added \setmoremathsizes and hooks to, e.g. \@xpt,
%             for support of bold Greek
%
%%ltg added this to try to get 12pt to come through
%\DeclareOption{12pt}{\renewcommand\@ptsize{2}}
%%end ltg

\def\@ptoptions{%
 \let\@elt\relax\@for\@tempa:=\@optionlist\do{%
  \expandafter\let\expandafter\@tempb\csname ds@\@tempa\endcsname
  \expandafter\let\expandafter\@tempc\csname ds@11pt\endcsname
  \ifx\@tempb\@tempc\else
   \expandafter\let\expandafter\@tempc\csname ds@12pt\endcsname
   \ifx\@tempb\@tempc\else\let\@tempb\relax\fi
   \fi
  \@tempb
  }%
 }%
%
% read in style file, but only process the pt size options
%
\def\@ptoptinput#1{%
 \let\@save@optionlist\@optionlist
 \let\@save@options\@options
 \let\@options\@ptoptions
 %
 \input #1
 %
 \let\@optionlist\@save@optionlist
 \let\@options\@save@options
 }%
%
% the <21 Feb 92> version of letter.sty requires:
\ifx\undefined\reset@font
 \def\reset@font{}%
 \fi
%
% Change LaTeX
%
% Add command to append tokens
\newtoks\@temptokenb
\long\def\appdef#1#2{%
 \ifx#1\undefined\let#1\@empty\fi
 \@temptokena\expandafter{#1}\@temptokenb{#2}%
 \edef#1{\the\@temptokena\the\@temptokenb}%
 }%
\long\def\prepdef#1#2{%
 \ifx#1\undefined\let#1\@empty\fi
 \@temptokena\expandafter{#1}\@temptokenb{#2}%
 \edef#1{\the\@temptokenb\the\@temptokena}%
 }%
% Discard contents of \box\@cclv at beginning of document
\appdef\document{{\output{\setbox\z@\box\@cclv}\endgraf\null\eject}}%
% Fix mark register expansion
\def\leftmark{\expandafter\@leftmark\botmark{}{}{}\@nil}%
\def\rightmark{\expandafter\@rightmark\firstmark{}{}{}\@nil}%
\def\@leftmark#1#2#3\@nil{#1}%
\def\@rightmark#1#2#3\@nil{#2}%
%
%\show\raggedright
\newskip\raggedglue
\raggedglue\z@ plus20\p@ minus\z@
\def\raggedright{%
 \let\\=\@centercr\@rightskip\raggedglue\rightskip
 \@rightskip\leftskip\z@\parindent\z@
 }%
%
\def\@centercr{%
 \ifhmode\unskip\else\@badcrerr\fi\@@par
 \@ifstar{\penalty\@M\@xcentercr}{\@xcentercr}%
 }%
%
\def\traceoutput{\tracingoutput2\showboxbreadth\maxdimen
 \showboxdepth\maxdimen}%
%
\newcount\@hour\newcount\@minute\chardef\@x10\chardef\@xv60
\def\@time{%
  \@minute\time\@hour\@minute\divide\@hour\@xv
  \ifnum\@hour<\@x 0\fi\the\@hour:%
  \multiply\@hour\@xv\advance\@minute-\@hour
  \ifnum\@minute<\@x 0\fi\the\@minute
  }%
%
% change \@array to allow \par to mean something within its scope
%
\def\@array [#1]#2{%
 \setbox\@arstrutbox\hbox{\vrule height\arraystretch\ht
  \strutbox depth\arraystretch\dp\strutbox width\z@}%
 \@mkpream{#2}%
 \edef\@preamble{\halign\noexpand\@halignto\bgroup\tabskip
  \z@\@arstrut\@preamble\tabskip\z@\cr}%
 \let\@startpbox\@@startpbox\let\@endpbox\@@endpbox
 \if#1t\vtop\else\if#1b\vbox\else\vcenter\fi\fi
 \bgroup
  %\let\par\relax
  \let\@sharp##
  \let\protect\relax
  \lineskip\z@\baselineskip\z@
  \@preamble
 }%
%
% Expands to hex digit corresponding to the value of the argument
%
\def\hexnumber@#1{\ifnum#1<10 \number#1\else
 \ifnum#1=10 A\else\ifnum#1=11 B\else\ifnum#1=12 C\else
 \ifnum#1=13 D\else\ifnum#1=14 E\else\ifnum#1=15 F\fi\fi\fi\fi\fi\fi\fi}%
%
% define command to set more math sizes.
% Styles like Greekbf will hook in here.
%
\def\setmoremathsizes#1#2#3{}%
%
% define size switch addenda
%  Note: these choices agree with those in lfonts.tex, even if incorrect.
%
\prepdef\@vpt{\setmoremathsizes{fiv}{fiv}{fiv}}%
\prepdef\@vipt{\setmoremathsizes{six}{six}{six}}%
\prepdef\@viipt{\setmoremathsizes{sev}{fiv}{fiv}}%
\prepdef\@viiipt{\setmoremathsizes{egt}{six}{fiv}}%
\prepdef\@ixpt{\setmoremathsizes{nin}{six}{fiv}}%
\prepdef\@xpt{\setmoremathsizes{ten}{sev}{fiv}}%
\prepdef\@xipt{\setmoremathsizes{elv}{egt}{six}}%
\prepdef\@xiipt{\setmoremathsizes{twl}{egt}{six}}%
\prepdef\@xivpt{\setmoremathsizes{frtn}{ten}{sev}}%
\prepdef\@xviipt{\setmoremathsizes{svtn}{twl}{ten}}%
\prepdef\@xxpt{\setmoremathsizes{twty}{frtn}{twl}}%
\prepdef\@xxvpt{\setmoremathsizes{twty}{twty}{svtn}}%
%
% The \newfield command defines (like \newenvironment) a user syntax:
%
%   \newfield{foo}
%
% lets you write
%
%   \begin{foo}...\end{foo}
%
% but differs from \newenvironment in that TeX parses the entire content
% of the field and stores it in a macro \the@foo, and then executes \@do@foo.
%
% This means that the content of the field is actually more like an argument
% than the content of an environment. So \verb will not necessarily work
% within a field, and neither will \index. Caveat emptor.
%
% The default procedure for a field is to process its argument within a
% group.  If you want a field to simply store its data away, define its
% procedure to be synonymous with \@empty, as illustrated below.
%
\long\def\@readenvir#1#2\end{%
 \appdef\envirsofar{#2}%
 \@ifnextchar\bgroup{\@checkenvir{#1}}{\@envirenderr}%
 }%
%
\def\@envirenderr{%
 \@latexerr{\string\end\space not followed by environment name}\@eha
 }%
%
\def\@checkenvir#1#2{%
 \def\@tempa{#1}\def\@tempb{#2}%
 \ifx\@tempa\@tempb
  \ifx\envirsofar\@blankspace\let\envirsofar\@empty\fi
  \expandafter\let\csname the@#1\endcsname\envirsofar
  \def\@tempa{\csname @do@#1\endcsname}%
  \else
  \appdef\envirsofar{\end{#2}}%
  \def\@tempa{\@readenvir{#1}}%
  \fi
 \@tempa
 }%
%
\def\newfield#1#2{%
 \expandafter\@ifdefinable\csname#1\endcsname{%
  \expandafter\def\csname#1\endcsname{%
   \endgroup\let\envirsofar\@empty\@readenvir{#1}%
   }%
  \expandafter\let\csname the@#1\endcsname\@empty
  \expandafter\ifx\csname @do@#1\endcsname\relax
   \expandafter\def\csname @do@#1\endcsname{{\csname the@#1\endcsname}}%
   \fi
  }%
 }%
%
\def\@blankspace{ }% SciWord's nil field
%
\def\letparBL{\def\par{\\}}%
\def\letparSP{\def\par{\ }}%
\def\letparQD{\def\par{\quad}}%
\def\letparSL{\def\par{\hbox to1em{\hfil/\hfil}}}%
%
% When \par is processed in the page head, gobble up the rest of the
% argument.
\def\@gobblepar#1\@empty{}%
%
% Physical page size after trim
\newdimen\trimwidth
\newdimen\trimheight
\newdimen\botmargin
\newdimen\marginpartotal
%
\def\adjustpagemargin{% adjust \oddsidemargin by \marginpartotal
 \marginpartotal\marginparwidth\advance\marginpartotal\marginparsep
 \advance\oddsidemargin\marginpartotal
 }%
%
\def\settextheight{% calculate textheight constrained by:
 \textheight\trimheight
 \advance\textheight-\topmargin
 \advance\textheight-\headheight
 \advance\textheight-\headsep
 \advance\textheight-\footskip
 \advance\textheight-\botmargin
 }%
%
\def\vcenterpagemargin{% calculate \topmargin constrained by:
 \topmargin\trimheight
 \advance\topmargin-\textheight
 \advance\topmargin-\headheight
 \advance\topmargin-\headsep
 \advance\topmargin-\footskip
 \divide\topmargin\tw@\botmargin\topmargin
 }%
%
\def\centerpagemargin{% calculate \oddsidemargin constrained by:
 \oddsidemargin\trimwidth
 \advance\oddsidemargin-\textwidth
 \advance\oddsidemargin-\marginparwidth
 \advance\oddsidemargin-\marginparsep
 \divide\oddsidemargin\tw@
 \evensidemargin\oddsidemargin
 \adjustpagemargin
 }%
%
\def\leftpagemargin{% calculate \oddsidemargin constrained by:
 \oddsidemargin\trimwidth
 \advance\oddsidemargin-\textwidth
 \advance\oddsidemargin-\marginparwidth
 \advance\oddsidemargin-\marginparsep
 \advance\oddsidemargin-\evensidemargin
 \adjustpagemargin
 }%


==> telescopes/acronym_tel.tex <==
\begin{flushleft}
\begin{tabular} {ll}
\textbf{AHWP} & Achromatic Half Wave Plate \\
\textbf{AR} & Anti-Reflection \\
\textbf{AZ} & AZimuth \\
\textbf{CFRP} &  Carbon Fiber Reinforced Polymer \\
%\textbf{CLASS} & Cosmology Large Angular Scale Surveyor \\
\textbf{EL} & ELevation \\
\textbf{FOV} & Field Of View \\
\textbf{FWHM} & Full Width Half Maximum \\
\textbf{HDPE} & High-Density PolyEthylene\\
\textbf{HF} & High Frequency \\
\textbf{HWP} & Half Wave Plate\\
\textbf{IR} & InfraRed \\
%\textbf{LHE} & Liquid Helium \\
\textbf{OMT} & Ortho-Mode Transducer \\
\textbf{PTFE} & PolyTetraFluoroEthylene \\
\textbf{UHMWPE} & Ultra-High Molecular Weight PolyEthylene \\
\textbf{VPM} & Variable Polarization Modulator \\
\end{tabular}
\end{flushleft}

